Evaluating Fuzz Testing

Fuzz testing has enjoyed great success at discovering security critical bugs in real software. Recently, researchers have devoted significant effort to devising new fuzzing techniques, strategies, and algorithms. Such new ideas are primarily evaluated experimentally so an important question is: What experimental setup is needed to produce trustworthy results? We surveyed the recent research literature and assessed the experimental evaluations carried out by 32 fuzzing papers. We found problems in every evaluation we considered. We then performed our own extensive experimental evaluation using an existing fuzzer. Our results showed that the general problems we found in existing experimental evaluations can indeed translate to actual wrong or misleading assessments. We conclude with some guidelines that we hope will help improve experimental evaluations of fuzz testing algorithms, making reported results more robust.

==> intro.tex <==

\section{Introduction}

\sw{Outline. Fuzzing is popular and important. Many techniques
have been developed. The challenge is to understand when and why
a particular solution works, so appropriate techniques can be used under
different scenarios. This goal can be achieved through rigorous empirical
study of fuzzing techniques. Unfortunately, most fuzzing evaluations failed
this task (e.g., ...). This paper presents the guideline to rigorously evaluate
fuzzing techniques, and we have tested the guide by actually studying several
popular fuzzing techniques. What we did/contributions: 1. A general algorithm
that integrates recently proposed fuzzing techniques. It makes it easier to compare
against different techniques in theory as well as empirically under unified settings.
2. We present guidance with a focus on statistical significance and other aspects
to consider in fuzzing evaluation (e.g., benchmarking, seed selection). We demonstrate
the importance to follow this guidance in future fuzzing evaluation by
studying several state-of-the-art fuzzers.}

When it comes to software development, simply ``making it work" is no longer sufficient. Today's software is constantly bombarded with untrusted inputs, and is under threat from a wide array of people and groups, ranging from small-scale hackers motivated by thrills or money to entire nation-states motivated by their political interests. Security and reliability are not optional features to be tacked on as afterthoughts; they are necessary in order to avoid putting users and their data at risk. Unfortunately, far too many programmers still do treat the robustness of their code as an afterthought.
In many cases, security is such an afterthought that the programmers themselves aren't the ones finding the bugs. Instead, bugs are often discovered by outside researchers after the program has already been released. As a result, fatal bugs do not get fixed until some time following their identification in the wild. Worst of all are situations when black-hat hackers are among the first to discover a bug. Then these malicious actors are able to exploit the vulnerability with impunity before it even lands on the programmer's radar. These bugs, called zero-days, are the most insidious type of bugs.
Properly writing modern-day software requires a real shift in how it is developed. Software robustness needs to be a preemptive goal. That goal, unfortunately, is not as simple as ordering programmers to write better code. Improving the way programmers write and audit code is an important first step, and secure coding practices should always be encouraged, but these solutions can only go so far. Scaling manual analysis up to large, complex projects with thousands or even millions of lines of code quickly becomes infeasible. Automated tools are now an indispensable part of finding vulnerabilities, which developers have already begun to and will need to continue adopting.

One of the most popular automated testing techniques is software fuzz testing (fuzzing). Its use in the information security field, particularly to validate mass-market software like Google Chrome \sw{reference}, has risen greatly in the past several years. As security becomes more of an essential consideration for developers and testers, the use of fuzzing is bound to increase, and along with it, the demand for more efficient and effective fuzzing. This has resulted in a significant amount of new fuzzing research, largely to improve the technique's performance \sw{references}.
The initial concept of fuzzing, feeding random inputs to a program and seeing if they cause crashes, has been greatly expanded upon over the years. One of the major innovations was coverage-based greybox fuzzing (CGF) \sw{reference}, popularized by the well-known fuzzer AFL \sw{reference}. CGF is able to detect whether certain inputs trigger new paths and guide the fuzzer towards generating inputs that expose new paths. In essence, a coverage-based fuzzer evolves its inputs towards increased program coverage.
On top of CGF fuzzers, researchers have built further new techniques. In Section \ref{background}, we systematically summarized these additions, which help the fuzzer uncover new paths that are difficult to reach solely through random input mutations. As part of our attempt to explain the mechanics coverage-based fuzzing and the various modifications made to it, we present a generic pseudocode overview of the algorithm behind standard CGF fuzzers. The algorithm is broken up into a series of modular functions, whose inner-workings are altered by CGF modifications. This allows us to describe research in the field much more simply, by highlighting only the differences with standard CGF and showing how they fit into the overall fuzzing process.

Improving on standard CGF is one of the most active areas of inquiry in fuzzing research \sw{references}.
The research into how fuzzing can be improved gives way to a more fundamental question: what makes a fuzzing algorithm effective or ineffective at finding bugs in certain types of programs? We do not claim to have an answer to this question, but the first step in answering it is gathering data on how different fuzzers perform on a variety of benchmark programs. Research in the field contributes towards solving that broader question. But as a review of computer science research indicates \sw{which one?}, existing work is producing results without statistical validity. Fuzzing techniques are often evaluated based on one trial (or very few) \sw{references}, fail to use statistical tests \sw{references}, and/or do not compare results to baselines \sw{references}.

In this paper, we provide rules on rigorous evaluating fuzzing techniques. Following these principles, our experiments are repeated in enough trials to be statistically-significant, and the data is analyzed using confidence intervals and hypothesis tests. Even more uniquely, we adopt a non-coverage-guided fuzzer (AFL with no instrumentation analysis) as a baseline in order to test the assumption of how essential CGF actually is, and to determine if there are situations in which coverage guidance becomes more or less useful. Finally, we introduce a broader suite of benchmark programs on which the fuzzers are tested. Currently, there is no standard set of programs used for fuzzing research evaluation, which hampers the comparability of different CGF modifications. Most papers use different programs from one another, or even neglect real-world programs in favor of artificial sets like CGC or LAVA. We adopt a benchmark suite that incorporates programs from several research papers, giving us a broader common-ground of programs to test on. This suite also gives us tests that are as close to realistic as possible, and cover a greater set of program behaviors, since we use multiple classes of real-world programs (ELF parsers, file converters, etc.) as benchmarks. 

As such, a secondary goal that arises in our paper is rechecking claims made by past papers with a more solid testing methodology. Not only does this test reproducibility (a tenet of modern science), but it also determines whether conclusions about fuzzers derived from a limited set of benchmarks are applicable to other programs.\sw{summarize the results.}

In summary, this paper contributes the following:

A pseudocode outline of how coverage-based fuzzing works.

Principles on evaluating fuzzing techniques: multiple trials, statistical tests, random baselines (``dumb" fuzzer), and consistent benchmarks.

Testing of fuzzer assumptions often taken for granted, such as the importance of coverage-based fuzzing and whether a CGF should be seeded with valid inputs.

Rechecking of claims from past research, using our improved methodology.


==> paper/intro.tex <==

\section{Introduction}

\sw{Outline. Fuzzing is popular and important. Many techniques
have been developed. The challenge is to understand when and why
a particular solution works, so appropriate techniques can be used under
different scenarios. This goal can be achieved through rigorous empirical
study of fuzzing techniques. Unfortunately, most fuzzing evaluations failed
this task (e.g., ...). This paper presents the guideline to rigorously evaluate
fuzzing techniques, and we have tested the guide by actually studying several
popular fuzzing techniques. What we did/contributions: 1. A general algorithm
that integrates recently proposed fuzzing techniques. It makes it easier to compare
against different techniques in theory as well as empirically under unified settings.
2. We present guidance with a focus on statistical significance and other aspects
to consider in fuzzing evaluation (e.g., benchmarking, seed selection). We demonstrate
the importance to follow this guidance in future fuzzing evaluation by
studying several state-of-the-art fuzzers.}

When it comes to software development, simply ``making it work" is no longer sufficient. Today's software is constantly bombarded with untrusted inputs, and is under threat from a wide array of people and groups, ranging from small-scale hackers motivated by thrills or money to entire nation-states motivated by their political interests. Security and reliability are not optional features to be tacked on as afterthoughts; they are necessary in order to avoid putting users and their data at risk. Unfortunately, far too many programmers still do treat the robustness of their code as an afterthought.
In many cases, security is such an afterthought that the programmers themselves aren't the ones finding the bugs. Instead, bugs are often discovered by outside researchers after the program has already been released. As a result, fatal bugs do not get fixed until some time following their identification in the wild. Worst of all are situations when black-hat hackers are among the first to discover a bug. Then these malicious actors are able to exploit the vulnerability with impunity before it even lands on the programmer's radar. These bugs, called zero-days, are the most insidious type of bugs.
Properly writing modern-day software requires a real shift in how it is developed. Software robustness needs to be a preemptive goal. That goal, unfortunately, is not as simple as ordering programmers to write better code. Improving the way programmers write and audit code is an important first step, and secure coding practices should always be encouraged, but these solutions can only go so far. Scaling manual analysis up to large, complex projects with thousands or even millions of lines of code quickly becomes infeasible. Automated tools are now an indispensable part of finding vulnerabilities, which developers have already begun to and will need to continue adopting.

One of the most popular automated testing techniques is software fuzz testing (fuzzing). Its use in the information security field, particularly to validate mass-market software like Google Chrome \sw{reference}, has risen greatly in the past several years. As security becomes more of an essential consideration for developers and testers, the use of fuzzing is bound to increase, and along with it, the demand for more efficient and effective fuzzing. This has resulted in a significant amount of new fuzzing research, largely to improve the technique's performance \sw{references}.
The initial concept of fuzzing, feeding random inputs to a program and seeing if they cause crashes, has been greatly expanded upon over the years. One of the major innovations was coverage-based greybox fuzzing (CGF) \sw{reference}, popularized by the well-known fuzzer AFL \sw{reference}. CGF is able to detect whether certain inputs trigger new paths and guide the fuzzer towards generating inputs that expose new paths. In essence, a coverage-based fuzzer evolves its inputs towards increased program coverage.
On top of CGF fuzzers, researchers have built further new techniques. In Section \ref{background}, we systematically summarized these additions, which help the fuzzer uncover new paths that are difficult to reach solely through random input mutations. As part of our attempt to explain the mechanics coverage-based fuzzing and the various modifications made to it, we present a generic pseudocode overview of the algorithm behind standard CGF fuzzers. The algorithm is broken up into a series of modular functions, whose inner-workings are altered by CGF modifications. This allows us to describe research in the field much more simply, by highlighting only the differences with standard CGF and showing how they fit into the overall fuzzing process.

Improving on standard CGF is one of the most active areas of inquiry in fuzzing research \sw{references}.
The research into how fuzzing can be improved gives way to a more fundamental question: what makes a fuzzing algorithm effective or ineffective at finding bugs in certain types of programs? We do not claim to have an answer to this question, but the first step in answering it is gathering data on how different fuzzers perform on a variety of benchmark programs. Research in the field contributes towards solving that broader question. But as a review of computer science research indicates \sw{which one?}, existing work is producing results without statistical validity. Fuzzing techniques are often evaluated based on one trial (or very few) \sw{references}, fail to use statistical tests \sw{references}, and/or do not compare results to baselines \sw{references}.

In this paper, we provide rules on rigorous evaluating fuzzing techniques. Following these principles, our experiments are repeated in enough trials to be statistically-significant, and the data is analyzed using confidence intervals and hypothesis tests. Even more uniquely, we adopt a non-coverage-guided fuzzer (AFL with no instrumentation analysis) as a baseline in order to test the assumption of how essential CGF actually is, and to determine if there are situations in which coverage guidance becomes more or less useful. Finally, we introduce a broader suite of benchmark programs on which the fuzzers are tested. Currently, there is no standard set of programs used for fuzzing research evaluation, which hampers the comparability of different CGF modifications. Most papers use different programs from one another, or even neglect real-world programs in favor of artificial sets like CGC or LAVA. We adopt a benchmark suite that incorporates programs from several research papers, giving us a broader common-ground of programs to test on. This suite also gives us tests that are as close to realistic as possible, and cover a greater set of program behaviors, since we use multiple classes of real-world programs (ELF parsers, file converters, etc.) as benchmarks. 

As such, a secondary goal that arises in our paper is rechecking claims made by past papers with a more solid testing methodology. Not only does this test reproducibility (a tenet of modern science), but it also determines whether conclusions about fuzzers derived from a limited set of benchmarks are applicable to other programs.\sw{summarize the results.}

In summary, this paper contributes the following:

A pseudocode outline of how coverage-based fuzzing works.

Principles on evaluating fuzzing techniques: multiple trials, statistical tests, random baselines (``dumb" fuzzer), and consistent benchmarks.

Testing of fuzzer assumptions often taken for granted, such as the importance of coverage-based fuzzing and whether a CGF should be seeded with valid inputs.

Rechecking of claims from past research, using our improved methodology.


==> paper/related.tex <==

Fuzzing seeks to expose a program to a variety of inputs that are designed to execute interesting paths and reveal bugs (usually crashes). By sending the right inputs, a fuzzer can force a program to exercise unintended paths, revealing new bugs. Depending on the level of knowledge that the fuzzer has about the program and its input format, these inputs can be chosen randomly, systematically, or somewhere in between.

At their most basic, fuzzers simply generate random inputs. For programs requiring structured input, it would be nearly impossible for random inputs to be accepted, so random fuzzers actually tend to start from ``seed" inputs known to be valid as a template. They make random mutations to this seed, such as flipping bits or inserting/deleting blocks, feed it to the program, and observe whether or not the program crashes.

Mutation-based black-box fuzzing like this makes generating inputs very fast and scalable, but its effectiveness is limited. With no knowledge of the program's execution, the feedback the fuzzer gets is limited to whether or not the program crashed, making it hard to determine how promising an input is - many fuzzers apply evolutionary algorithms to mutate their inputs, which depend on this kind of ``fitness" assessment.

Coverage-based greybox fuzzing (CGF) adds instrumentation to a program binary, allowing its control flow to be monitored. That way, the fuzzer can get some idea of which paths the program traversed in response to an input, which helps it evaluate that input and adapt. To some degree, CGF even allows a fuzzer to work without a seed, since it can often use coverage information to learn the input structure. For instance, take a file format with a magic number at the beginning. Starting from an empty seed, the fuzzer would begin to randomly add and replace bytes. Initially, these inputs would all be rejected, since the magic number would not be correct. But as soon as a random mutation produced the correct magic number, the program would move past the initial check and into deeper paths. Coverage analysis would reveal that a new path had been reached, allowing the evolutionary algorithm to flag that input as a useful seed to generate further inputs from. Further inputs would then all pass the magic number check, allowing the CGF to repeat its discovery of other parts of the file format.
Laid out in pseudocode, the algorithm for a CGF is roughly as follows: \sw{migrate the code here, and discuss the algorithm following the lines. Say more on its generality.}

This pseudocode is inspired by the work of the AFLFast authors \sw{reference}, who devised a similar code sequence to explain how CGFs work and describe which functions they modified in AFLFast. (AFLFast will be discussed further below.)

Before running, the fuzzer gets a collection of seeds using GetSeeds() and adds it to a queue (T). If there are no seeds provided as input, it starts off with an empty seed.
In may cases, the fuzzer will have a pre-processing step that analyzes the program. This routine is encapsulated in AnalyzeProgram(). AFL, for instance, verifies that instrumentation is present. Other fuzzers (see below) might do more involved pre-fuzzing analysis.

The fuzzer run then starts until a timeout (e.g. 24 hours) occurs. A seed is pulled off the queue using ChooseNext(), and with AssignEnergy() it gets an ``energy" value: the number of mutations to produce from the seed. Until the seed?s energy runs out, it gets mutated (MutateInput()) and then the program is tested with that mutated seed (TestInput()). If the program crashes as a result of the input, it gets triaged to determine whether it?s unique or previously found (TriageCrash()) and then added to the list of crashing inputs (Tcrash). If the program didn't crash, but the fuzzer?s evolutionary algorithm considers the input worth keeping (IsInteresting()), the crashing input is put on the queue of seeds to fuzz next.

At the same time, the fuzzer tracks how many mutations it has gone through without generating any new interesting inputs. If it goes too long (THRESHOLD) without doing so or runs out of seeds entirely, the fuzzer is considered ``stuck". Depending on the fuzzer, it now has to do something to get itself unstuck. Some fuzzers are able to use previously-found interesting seeds to derive new interesting seeds, often by invoking a white-box analyzer (see below); this is encapsulated in the ResolveStuck() function. Otherwise, the fuzzer will simply take the seeds that were provided to the fuzzer at the very beginning and try another run.

Recent research into fuzzing typically focuses on increasing performance by either refining the pathfinding or improving the input generation. Each paper changes a particular set of functions in the above pseudocode, while maintaining the overall structure.
	
Pham, et. al. devised AFLFast, a modified AFL designed to expose uncommon paths earlier in a fuzzing run \cite{}. By modeling the fuzzing run as a Markov chain, they gain an insight into why running less frequent paths is so difficult: the probability distribution of exercising program paths quickly settles down into a distribution that gives some paths very high probability density and others very low probability density. As a result, the less-likely paths may become prohibitively unlikely to ever get executed. This is exacerbated by how AFL assigns seed energy: it gives constant energy to all seeds, which leads to too few inputs being generated from seeds that exercise low-density paths (which need more exposure) and vice-versa for high-density.
AFLFast modifies ChooseNext() to pick seeds that have been chosen less in the past and lead to paths with lower probability density. Its AssignEnergy() makes a seed?s energy inversely proportional to the path probability density (so lower probability paths are fuzzed more) and exponentially proportional to how many times times the seed has been chosen. Tested on GNU binutils applications, AFLFast found more unique crashes in less time than AFL. A team using it in the the DARPA Cyber Grand Challenge (CGC) won 2nd place for number of bugs found.

The Driller tool \cite{} combines fuzzing and symbolic execution, developing a fuzzer that invokes concolic execution when it is unable to expose new paths (gets stuck). Symbolic execution is a white-box technique which analyzes the program internals to systematically construct useful inputs. Programs are comprised of a finite number of paths, whose conditions for executing usually depend on the input data. In principle, there is a set of input constraints required to execute each path in a program. A symbolic executor represents inputs as symbols, propagates them through the program, and figures out these conditions. Building on this concept is concolic execution, which runs symbolic execution with a concrete input. It dynamically solves the constraints to make new inputs and trigger new paths as the program is tested.
The above caveat of ``In principle" is important to keep in mind. While theoretically possible to cover every part of the program with symbolic execution, it is not feasible to enumerate every single path. Each if-else fork in the road causes the number of paths to grow exponentially, and loops make that even worse. This problem, called path explosion, prevents symbolic execution from matching the scalability of fuzzing with complex real-world programs. It can, however, be incorporated as a ?helper? for certain fuzzing scenarios.
Driller's key insight is drawing a distinction between general and specific inputs to a program. General inputs (e.g. names) are open-ended and can take on a wide range of potential values, while specific inputs (e.g. magic numbers or commands) must match a limited set of values. Fuzzers, with their random mutations, are well-suited to explore general input, but they would be hard-pressed to pass a check for specific input. Symbolic execution is the perfect tool to solve specific checks, but the path explosion problem inhibits its use outside of this limited context. So Driller leverages the strengths and mitigates the weaknesses of both: fuzzing is the primary mode of exploration, and concolic execution is used to pass specific checks when the fuzzer gets stuck and allow it to continue fuzzing.
As such, the coverage-based fuzzer core of AFL remains intact, and is simply augmented with a symbolic executor for handling when the fuzzer gets stuck. ResolveStuck() invokes a symbolic executor (specifically angr). It takes an interesting seed input, feeds the input to angr to get deeper into the program, and returns a new seed that does so. The fuzzer (as per the pseudocode above) then uses these new seeds from ResolveStuck() to continue fuzzing normally.
Driller?s results are promising, though limited. The authors tested Driller on 126 programs from the CGC, comparing it against a fuzzer (AFL) and symbolic executor as baselines. The symbolic executor only managed to crash 16 programs. The fuzzer crashed 68 programs, and became unable to expose any new paths in 41 programs. With Driller, these 41 programs ended up invoking the concolic executor, which led to 9 additional crashes - a 12\% improvement over AFL. Driller found all the fuzzer?s bugs, all the symbolic executor?s bugs, and 6 bugs found by neither. However, Driller?s improvement to fuzzing is marginal: in 32 of the 41 programs that got stuck with AFL, Driller failed to find any deeper crashes.

The VUzzer \cite{} team highlighted some of the shortcomings of Driller and decided that incorporating symbolic execution was not an appropriate way to improve fuzzers. Instead, they opted to make a fuzzer with better input generation. To match the required input format, their fuzzer (VUzzer) is able to figure out specific required values like Driller does, but without needing symbolic execution. And to encourage deeper code execution, VUzzer prioritizes harder-to-reach paths. Each basic block in the program has a weight - higher weights mean that it should be prioritized to run. Uncommon blocks get higher weights, and error code gets the lowest weights of all.
At the beginning of its run, in AnalyzeProgram(), VUzzer collects the necessary information to build valid inputs and assess fitness. It uses dynamic taint analysis (DTA) to detect x86 cmp instructions that depend on input data, determining which of the input bytes must match specific values. VUzzer then builds a control flow graph of basic blocks in the program, calculating the probabilities of reaching the blocks and giving less common blocks higher weight. Error blocks, detected by seeing which blocks are executed by totally random input but not by known valid input, are given negative weights.
The core of VUzzer is an evolutionary input mutation algorithm. An input's fitness is calculated as the weighted sum of how many basic block executions occur, so input that runs more high-priority paths is considered best. Each iteration, the most ?fit? inputs (as assessed by the IsInteresting() function) are preserved for mutation. In the MutateInput() function, these inputs are crossed over and mutated as in a normal genetic algorithm, with the required bytes found by DTA filled in to ensure the input is valid. TestInput() continually updates VUzzer?s internal state as new inputs are tested. Which blocks are considered to be error handling code is an assessment that gets updated with each new run. Also, if inputs expose previously-unexecuted basic blocks, DTA is performed on those inputs to capture their essential traits.
VUzzer has an acute limitation on interactive binaries (like many found in CGC), but it far outperformed AFL in terms of bug finding on the LAVA test suite and many real-world Linux file conversion applications, often by more than double the effectiveness.

While the preceding papers optimized fuzzer path traversal by direct modification to the fuzzer core, other research leaves the fuzzer core intact and focuses on seed selection. In effect, the only modifications that the following papers make to the pseudocode is to the GetSeeds() function. As explained before, coverage-based greybox fuzzing somewhat mitigates the requirement of having seeds, since some of the input format can be ?learned? through coverage analysis. Our paper assesses how much seeds matter with a CGF fuzzer, so understanding the research into seed selection is quite important.

Rebert, et al. took a somewhat more theoretical look at seed selection \cite{}. Their experiments were done with BFF, which is a black-box fuzzer and thus not directly applicable to our CGF research. However, the paper still raises some interesting results, which deserve to be tested on a coverage-based fuzzer to see if they still occur.
From a collection of valid inputs to a program, we can draw a set of seeds for the fuzzer. However, different seed sets will vary in their effectiveness at finding bugs. Without any knowledge of how the sets perform, it would be fairest to simply pick a random set. However, if it's known in advance which code paths each seed triggers, we can apply the (NP-complete) set cover problem to select a set of seeds that maximizes code coverage.
The paper authors compared random selection against various solutions to the set cover problem. A standard unweighted minimum set cover algorithm ended up being the most effective (in terms of bug finding) deterministic way to pick a seed set. Interesting, however, is that with enough seeds, a random set approaches optimal bug finding performance, and even outperforms some set cover algorithms. With 10 seeds, a random set reaches roughly half of optimal bug finding. By 35 seeds, it?s closer to 2/3 of the optimal bug finding performance.
That random seed selection could be nearly as effective as deterministic selection is quite noteworthy. It provides a modicum of justification for generating the seed sets in our experiments with random selection; but as noted earlier, the results in this paper might not apply to coverage-based fuzzers such as AFL.


==> related.tex <==

Fuzzing seeks to expose a program to a variety of inputs that are designed to execute interesting paths and reveal bugs (usually crashes). By sending the right inputs, a fuzzer can force a program to exercise unintended paths, revealing new bugs. Depending on the level of knowledge that the fuzzer has about the program and its input format, these inputs can be chosen randomly, systematically, or somewhere in between.

At their most basic, fuzzers simply generate random inputs. For programs requiring structured input, it would be nearly impossible for random inputs to be accepted, so random fuzzers actually tend to start from ``seed" inputs known to be valid as a template. They make random mutations to this seed, such as flipping bits or inserting/deleting blocks, feed it to the program, and observe whether or not the program crashes.

Mutation-based black-box fuzzing like this makes generating inputs very fast and scalable, but its effectiveness is limited. With no knowledge of the program's execution, the feedback the fuzzer gets is limited to whether or not the program crashed, making it hard to determine how promising an input is - many fuzzers apply evolutionary algorithms to mutate their inputs, which depend on this kind of ``fitness" assessment.

Coverage-based greybox fuzzing (CGF) adds instrumentation to a program binary, allowing its control flow to be monitored. That way, the fuzzer can get some idea of which paths the program traversed in response to an input, which helps it evaluate that input and adapt. To some degree, CGF even allows a fuzzer to work without a seed, since it can often use coverage information to learn the input structure. For instance, take a file format with a magic number at the beginning. Starting from an empty seed, the fuzzer would begin to randomly add and replace bytes. Initially, these inputs would all be rejected, since the magic number would not be correct. But as soon as a random mutation produced the correct magic number, the program would move past the initial check and into deeper paths. Coverage analysis would reveal that a new path had been reached, allowing the evolutionary algorithm to flag that input as a useful seed to generate further inputs from. Further inputs would then all pass the magic number check, allowing the CGF to repeat its discovery of other parts of the file format.
Laid out in pseudocode, the algorithm for a CGF is roughly as follows: \sw{migrate the code here, and discuss the algorithm following the lines. Say more on its generality.}

This pseudocode is inspired by the work of the AFLFast authors \sw{reference}, who devised a similar code sequence to explain how CGFs work and describe which functions they modified in AFLFast. (AFLFast will be discussed further below.)

Before running, the fuzzer gets a collection of seeds using GetSeeds() and adds it to a queue (T). If there are no seeds provided as input, it starts off with an empty seed.
In may cases, the fuzzer will have a pre-processing step that analyzes the program. This routine is encapsulated in AnalyzeProgram(). AFL, for instance, verifies that instrumentation is present. Other fuzzers (see below) might do more involved pre-fuzzing analysis.

The fuzzer run then starts until a timeout (e.g. 24 hours) occurs. A seed is pulled off the queue using ChooseNext(), and with AssignEnergy() it gets an ``energy" value: the number of mutations to produce from the seed. Until the seed?s energy runs out, it gets mutated (MutateInput()) and then the program is tested with that mutated seed (TestInput()). If the program crashes as a result of the input, it gets triaged to determine whether it?s unique or previously found (TriageCrash()) and then added to the list of crashing inputs (Tcrash). If the program didn't crash, but the fuzzer?s evolutionary algorithm considers the input worth keeping (IsInteresting()), the crashing input is put on the queue of seeds to fuzz next.

At the same time, the fuzzer tracks how many mutations it has gone through without generating any new interesting inputs. If it goes too long (THRESHOLD) without doing so or runs out of seeds entirely, the fuzzer is considered ``stuck". Depending on the fuzzer, it now has to do something to get itself unstuck. Some fuzzers are able to use previously-found interesting seeds to derive new interesting seeds, often by invoking a white-box analyzer (see below); this is encapsulated in the ResolveStuck() function. Otherwise, the fuzzer will simply take the seeds that were provided to the fuzzer at the very beginning and try another run.

Recent research into fuzzing typically focuses on increasing performance by either refining the pathfinding or improving the input generation. Each paper changes a particular set of functions in the above pseudocode, while maintaining the overall structure.
	
Pham, et. al. devised AFLFast, a modified AFL designed to expose uncommon paths earlier in a fuzzing run \cite{}. By modeling the fuzzing run as a Markov chain, they gain an insight into why running less frequent paths is so difficult: the probability distribution of exercising program paths quickly settles down into a distribution that gives some paths very high probability density and others very low probability density. As a result, the less-likely paths may become prohibitively unlikely to ever get executed. This is exacerbated by how AFL assigns seed energy: it gives constant energy to all seeds, which leads to too few inputs being generated from seeds that exercise low-density paths (which need more exposure) and vice-versa for high-density.
AFLFast modifies ChooseNext() to pick seeds that have been chosen less in the past and lead to paths with lower probability density. Its AssignEnergy() makes a seed?s energy inversely proportional to the path probability density (so lower probability paths are fuzzed more) and exponentially proportional to how many times times the seed has been chosen. Tested on GNU binutils applications, AFLFast found more unique crashes in less time than AFL. A team using it in the the DARPA Cyber Grand Challenge (CGC) won 2nd place for number of bugs found.

The Driller tool \cite{} combines fuzzing and symbolic execution, developing a fuzzer that invokes concolic execution when it is unable to expose new paths (gets stuck). Symbolic execution is a white-box technique which analyzes the program internals to systematically construct useful inputs. Programs are comprised of a finite number of paths, whose conditions for executing usually depend on the input data. In principle, there is a set of input constraints required to execute each path in a program. A symbolic executor represents inputs as symbols, propagates them through the program, and figures out these conditions. Building on this concept is concolic execution, which runs symbolic execution with a concrete input. It dynamically solves the constraints to make new inputs and trigger new paths as the program is tested.
The above caveat of ``In principle" is important to keep in mind. While theoretically possible to cover every part of the program with symbolic execution, it is not feasible to enumerate every single path. Each if-else fork in the road causes the number of paths to grow exponentially, and loops make that even worse. This problem, called path explosion, prevents symbolic execution from matching the scalability of fuzzing with complex real-world programs. It can, however, be incorporated as a ?helper? for certain fuzzing scenarios.
Driller's key insight is drawing a distinction between general and specific inputs to a program. General inputs (e.g. names) are open-ended and can take on a wide range of potential values, while specific inputs (e.g. magic numbers or commands) must match a limited set of values. Fuzzers, with their random mutations, are well-suited to explore general input, but they would be hard-pressed to pass a check for specific input. Symbolic execution is the perfect tool to solve specific checks, but the path explosion problem inhibits its use outside of this limited context. So Driller leverages the strengths and mitigates the weaknesses of both: fuzzing is the primary mode of exploration, and concolic execution is used to pass specific checks when the fuzzer gets stuck and allow it to continue fuzzing.
As such, the coverage-based fuzzer core of AFL remains intact, and is simply augmented with a symbolic executor for handling when the fuzzer gets stuck. ResolveStuck() invokes a symbolic executor (specifically angr). It takes an interesting seed input, feeds the input to angr to get deeper into the program, and returns a new seed that does so. The fuzzer (as per the pseudocode above) then uses these new seeds from ResolveStuck() to continue fuzzing normally.
Driller?s results are promising, though limited. The authors tested Driller on 126 programs from the CGC, comparing it against a fuzzer (AFL) and symbolic executor as baselines. The symbolic executor only managed to crash 16 programs. The fuzzer crashed 68 programs, and became unable to expose any new paths in 41 programs. With Driller, these 41 programs ended up invoking the concolic executor, which led to 9 additional crashes - a 12\% improvement over AFL. Driller found all the fuzzer?s bugs, all the symbolic executor?s bugs, and 6 bugs found by neither. However, Driller?s improvement to fuzzing is marginal: in 32 of the 41 programs that got stuck with AFL, Driller failed to find any deeper crashes.

The VUzzer \cite{} team highlighted some of the shortcomings of Driller and decided that incorporating symbolic execution was not an appropriate way to improve fuzzers. Instead, they opted to make a fuzzer with better input generation. To match the required input format, their fuzzer (VUzzer) is able to figure out specific required values like Driller does, but without needing symbolic execution. And to encourage deeper code execution, VUzzer prioritizes harder-to-reach paths. Each basic block in the program has a weight - higher weights mean that it should be prioritized to run. Uncommon blocks get higher weights, and error code gets the lowest weights of all.
At the beginning of its run, in AnalyzeProgram(), VUzzer collects the necessary information to build valid inputs and assess fitness. It uses dynamic taint analysis (DTA) to detect x86 cmp instructions that depend on input data, determining which of the input bytes must match specific values. VUzzer then builds a control flow graph of basic blocks in the program, calculating the probabilities of reaching the blocks and giving less common blocks higher weight. Error blocks, detected by seeing which blocks are executed by totally random input but not by known valid input, are given negative weights.
The core of VUzzer is an evolutionary input mutation algorithm. An input's fitness is calculated as the weighted sum of how many basic block executions occur, so input that runs more high-priority paths is considered best. Each iteration, the most ?fit? inputs (as assessed by the IsInteresting() function) are preserved for mutation. In the MutateInput() function, these inputs are crossed over and mutated as in a normal genetic algorithm, with the required bytes found by DTA filled in to ensure the input is valid. TestInput() continually updates VUzzer?s internal state as new inputs are tested. Which blocks are considered to be error handling code is an assessment that gets updated with each new run. Also, if inputs expose previously-unexecuted basic blocks, DTA is performed on those inputs to capture their essential traits.
VUzzer has an acute limitation on interactive binaries (like many found in CGC), but it far outperformed AFL in terms of bug finding on the LAVA test suite and many real-world Linux file conversion applications, often by more than double the effectiveness.

While the preceding papers optimized fuzzer path traversal by direct modification to the fuzzer core, other research leaves the fuzzer core intact and focuses on seed selection. In effect, the only modifications that the following papers make to the pseudocode is to the GetSeeds() function. As explained before, coverage-based greybox fuzzing somewhat mitigates the requirement of having seeds, since some of the input format can be ?learned? through coverage analysis. Our paper assesses how much seeds matter with a CGF fuzzer, so understanding the research into seed selection is quite important.

Rebert, et al. took a somewhat more theoretical look at seed selection \cite{}. Their experiments were done with BFF, which is a black-box fuzzer and thus not directly applicable to our CGF research. However, the paper still raises some interesting results, which deserve to be tested on a coverage-based fuzzer to see if they still occur.
From a collection of valid inputs to a program, we can draw a set of seeds for the fuzzer. However, different seed sets will vary in their effectiveness at finding bugs. Without any knowledge of how the sets perform, it would be fairest to simply pick a random set. However, if it's known in advance which code paths each seed triggers, we can apply the (NP-complete) set cover problem to select a set of seeds that maximizes code coverage.
The paper authors compared random selection against various solutions to the set cover problem. A standard unweighted minimum set cover algorithm ended up being the most effective (in terms of bug finding) deterministic way to pick a seed set. Interesting, however, is that with enough seeds, a random set approaches optimal bug finding performance, and even outperforms some set cover algorithms. With 10 seeds, a random set reaches roughly half of optimal bug finding. By 35 seeds, it?s closer to 2/3 of the optimal bug finding performance.
That random seed selection could be nearly as effective as deterministic selection is quite noteworthy. It provides a modicum of justification for generating the seed sets in our experiments with random selection; but as noted earlier, the results in this paper might not apply to coverage-based fuzzers such as AFL.

